An online data analysis system of INTEGRAL telescope

During more than 17 years of operation in space INTEGRAL telescope has accumulated large data set that contains records of hard X-ray and soft gamma-ray astronomical sources. These data can be re-used in the context of multi-wavelength or multi-messenger studies of astronomical sources and have to be preserved on long time scales. We present a scientific validation of an interactive online INTEGRAL data analysis system for multi-wavelength studies of hard X-ray and soft gamma-ray sources. The online data analysis system generates publication-quality high-level data products: sky images, spectra and light-curves in response to user queries that define analysis parameters, such as source position, time and energy interval and binning. The data products can be requested via a web browser interface or via Application Programming Interface (API) available as a Python package. The analysis workflow organized to preserve and re-use various intermediate analysis products, ensuring that frequently requested results are available without delay. The platform can be deployed in any compatible infrastructure. We report the functionalities and performance of the online data analysis system by reproducing the benchmark INTEGRAL results on different types of sources, including bright steady and transient Galactic sources, and bright and weak variable extra-galactic sources. We compare the results obtained with the online data analysis system with previously published results on these sources. We consider the INTEGRAL online data analysis as a demonstrator of more general web-based "data analysis as a service" approach that provides a promising solution for preservation and maintenance of data analysis tools of astronomical telescopes on (multi)decade long time scales and facilitates combination of data in multi-wavelength and multi-messenger studies of astronomical sources.

==> Crab_scws.tex <==
\begin{table*}
\begin{tabular}{|l|l|l|l|l|}
\hline
ScW &Start &  Exposure & Flux & $\Gamma$\\
\hline
193000200010 & 2018-03-14 08:30:03 &FAILED&&\\
192800120010 & 2018-03-08 15:34:36 &1041&$7.7\pm 0.4$&$2.111\pm 0.015$\\
192700120010 & 2018-03-06 05:26:37 &2061&$7.3\pm 0.2$&$2.102\pm 0.011$\\
192500120010 & 2018-02-28 16:05:50 &1037&$7.8\pm 0.4$&$2.114\pm 0.015$\\
192100120010 & 2018-02-18 02:22:30 &1019&$7.8\pm 0.4$&$2.116\pm 0.016$\\
187700120010 & 2017-10-24 01:05:32 &1062&$6.2\pm 0.3$&$2.045\pm 0.014$\\
186700130010 & 2017-09-27 18:04:56 &FAILED&&\\
186600100010 & 2017-09-24 18:14:26 &FAILED&&\\
185700120010 & 2017-08-31 23:31:56 &NOSOURCE?&&\\
185600120010 & 2017-08-29 05:55:05 &1465&$6.9\pm 0.3$&$2.067\pm 0.012$\\
185000120010 & 2017-08-13 03:04:22 &1037&$7.7\pm 0.4$&$2.091\pm 0.015$ \\
180100120010 & 2017-04-04 23:40:02 &1090&$11.9\pm 0.6$&$2.194\pm 0.015$\\
179700520010 & 2017-03-26 07:44:55 &FAILED&&\\
179400120010 & 2017-03-17 07:26:14 &1053&$10.6\pm 0.6$&$2.170\pm 0.016$\\
178900640010 & 2017-03-05 08:39:33 &306&$12.2\pm 1.3$&$2.21\pm 0.03$\\
178500120010 & 2017-02-21 14:33:05 &2028&$10.4\pm 0.4$&$2.161\pm 0.011$\\
178400120010 & 2017-02-18 20:32:59 &FAILED&&\\
178100120010 & 2017-02-10 17:48:47 &1048&$9.7\pm 0.5$&$2.142\pm 0.015$\\
173600120010 & 2016-10-14 02:24:14 &1078&$10.1\pm 0.5$&$2.137\pm 0.014$\\
173300120010 & 2016-10-06 04:03:07 &1070&$8.8\pm 0.5$&$2.099\pm 0.014$\\
172800690010 & 2016-09-24 04:43:18 &1105&$9.4\pm 0.5$&$2.122\pm 0.014$\\
172400120010 & 2016-09-12 08:04:17 &2288&$10.0\pm 0.4$&$2.132\pm 0.010$\\
172300120010 & 2016-09-09 15:49:06 &2106&$11.4\pm 0.4$&$2.173\pm 0.010$\\
171900700010 & 2016-08-31 05:25:25 &1246&$9.5\pm 0.5$&$2.126\pm 0.012$\\
171500120010 & 2016-08-19 04:46:31 &1100&$10.7\pm 0.6$&$2.151\pm 0.014$\\
166700510010 & 2016-04-14 21:21:44 &497&$11.0\pm 0.9$&$2.15\pm 0.02$\\
166400120010 & 2016-04-05 14:56:18 &1104&$9.7\pm 0.5$&$2.109\pm 0.014$\\
166200120010 & 2016-03-31 11:34:40 &2251&$7.6\pm 0.3$&$2.047\pm 0.010$\\
166100120010 & 2016-03-28 19:52:03 &FAILED&&\\
165800120010 & 2016-03-20 15:55:10 &1083&$8.3\pm 0.4$&$2.064\pm 0.013$\\
165700680010 & 2016-03-19 10:54:24 &FAILED&&\\
165200120010 & 2016-03-04 15:40:03 &1102&$9.3\pm 0.5$&$2.093\pm 0.014$\\
164800220010 & 2016-02-23 09:38:30 &1087&$8.0\pm 0.4$&$2.063\pm 0.014$\\
164400120010 & 2016-02-12 09:25:18 &FAILED&&\\
159900120010 & 2015-10-15 23:16:19 &3326&$8.0\pm 0.2$&$2.047\pm 0.007$\\
159800120010 & 2015-10-13 04:00:17 &2054&$8.9\pm 0.3$&$2.069\pm 0.009$\\	
159700120010 & 2015-10-10 13:26:50 &1164&$9.6\pm 0.4$&$2.092\pm 0.012$\\
159300620010 & 2015-10-01 07:38:10 &1076&$9.5\pm 0.5$&$2.091\pm 0.013$\\
158900120010 & 2015-09-19 04:03:58 &1179&$9.3\pm 0.4$&$2.081\pm 0.012$\\
158100120010 & 2015-08-28 21:00:08 &1175&$0.8\pm 0.4$&$2.096\pm 0.012$\\
157700120010 & 2015-08-18 05:03:31 &1161&$9.7\pm 0.4$&$2.086\pm 0.012$\\
152800120010 & 2015-04-10 01:28:30 &1200&$9.1\pm 0.4$&$2.085 \pm 0.012$\\
152400120010 & 2015-03-30 06:53:35 &720&$8.7\pm 0.5$&$2.074\pm 0.016$\\	
152000120010 & 2015-03-19 15:37:48 &1224&$8.5\pm 0.4$&$2.066\pm 0.012$\\
151600120010 & 2015-03-09 07:59:21 &2403&$10.0\pm 0.3$&$2.107\pm 0.009$\\
151500120010 & 2015-03-06 11:24:59 &2431&$9.1\pm 0.3$&$2.083\pm 0.008$\\
150800120010 &  2015-02-15 18:15:03	&1149&$8.6\pm 0.4$&$2.064\pm 0.012$\\
150600680010 & 2015-02-12 10:20:47 &812&$8.6\pm 0.6$&$2.073\pm 0.017$\\
150500530010 & 2015-02-09 18:11:23 &FAILED&&\\
147200200010 & 2014-11-02 23:01:21 &1423&$9.5\pm 0.5$&$2.091\pm 0.015$\\
146800310010 & 2014-10-22 02:27:35 &1166&$8.8\pm 0.4$&$2.077\pm 0.012$\\
146600850010 & 2014-10-17 21:49:21 &1220&$8.1\pm 0.4$&$2.063\pm 0.012$ \\
146200120010 & 2014-10-03 19:16:42 &1344 &$7.9\pm 0.3$& $2.047 0.011$\\
146100120010 & 2014-09-30 18:27:52 &FAILED&&\\
145600380010 & 2014-09-16 20:34:17 &1167&$8.5\pm 0.4$&$2.061\pm 0.012$\\
145200540010 & 2014-09-05 18:28:27 &NO SoURCE&&\\
144700620010 & 2014-08-21 19:47:00 &1177&$9.3\pm 0.4$&$2.094\pm 0.012$\\
144400610010 & 2014-08-12 21:58:05 &1268&$8.0\pm 0.3$&$2.058\pm 0.012$\\
138700120010 & 2014-02-21 11:12:06 &1395&$8.3\pm 0.3$&$2.061\pm 0.010$\\
134200120010 & 2013-10-09 19:14:07 &1397&$8.8\pm 0.4$&$2.069\pm 0.011$\\
132800120010 & 2013-08-28 22:56:49 &1379&$8.4\pm 0.3$&$2.065\pm 0.011$\\
132700120010 & 2013-08-25 22:42:11 &1262&$8.5\pm 0.4$&$2.063\pm 0.011$\\
127800120010 & 2013-04-01 08:48:58 &1363&$8.6\pm 0.4$&$2.067\pm 0.011$\\
\hline
\end{tabular}
\end{table*}
\begin{table*}
\begin{tabular}{|l|l|l|l|l|}
\hline
ScW &Start &  Exposure & Flux & $\Gamma$\\
\hline
126900120010 & 2013-03-05 13:02:02 &1324&$8.4\pm 0.4$&$2.061\pm 0.012$\\
126800120010 & 2013-03-02 11:40:09 &1272&$8.5\pm 0.4$&$2.067\pm 0.012$\\
122100120010 & 2012-10-12 22:08:55 &1399&$7.7\pm 0.3$&$2.034 \pm 0.012$\\
121400440010 & 2012-09-23 05:47:26 &FAILED&&\\
116000120010 & 2012-04-13 11:41:56 &1403&$8.2\pm 0.3$&$2.055\pm 0.011$\\
115900120010 & 2012-04-10 10:32:40 &1304&$9.6\pm 0.4$&$2.091\pm 0.012$\\
114000190010 & 2012-02-13 21:43:16 &FAILED&&\\
109600120010 & 2011-10-04 23:11:58 &1277&$6.7\pm 0.4$&$2.005\pm 0.015$\\
108900120010 & 2011-09-14 02:12:51 &1438&$8.5\pm 0.3$&$2.067\pm 0.011$\\
102800780010 & 2011-03-17 07:19:36 &2324&$8.5\pm 0.3$&$2.076 \pm 0.010$\\
102700810010 & 2011-03-14 13:08:40 &2241&$8.8\pm 0.3$&$2.085\pm 0.009$\\	
102600770010 & 2011-03-11 07:58:51 &1954&$8.8\pm 0.3$&$2.086\pm 0.011$\\
102500930010 & 2011-03-08 12:33:23 &1451&$8.5\pm 0.5$&$2.079\pm 0.015$\\
102400830010 & 2011-03-05 13:33:16 &362&$8.8\pm 0.8$&$2.09\pm 0.03$\\
102300850010 & 2011-03-02 14:01:48 &1069&$9.1\pm 0.5$&$2.091\pm 0.015$\\
102200730010 & 2011-02-27 16:32:57 &1755&$9.3\pm 0.4$&$2.101\pm 0.013$\\
102100420010 & 2011-02-24 00:44:15 &1762&$7.8\pm 0.3$&$2.059\pm 0.012$\\
101900120010 & 2011-02-16 15:55:00 &1191&$8.6\pm 0.5$&$2.076\pm 0.015$\\
097000120010 & 2010-09-23 02:53:23 &938&$7.7\pm 0.4$&$2.036\pm 0.014$\\
096800120010 & 2010-09-17 03:53:38 &1266&$8.8\pm 0.5$&$2.072\pm 0.015$ \\
096700120010 & 2010-09-14 07:10:42 &1780&$8.2\pm 0.3$&$2.062\pm 0.009$\\
096600590010 & 2010-09-12 16:21:01 &NO SOURCE?&&\\
091700120010 & 2010-04-17 16:55:46 &2188&$7.8\pm 0.3$&$2.044\pm 0.010$\\
091600120010 & 2010-04-14 17:08:22 &2150 &$8.6\pm 0.3$&$2.078\pm 0.010$\\
091500120010 & 2010-04-11 17:23:03 &2151&$8.9\pm 0.3$&$2.088\pm 0.010$\\
091400120010 & 2010-04-08 17:34:13 &FAILED&&\\
091200420010 & 2010-04-03 20:29:01 &2266&$9.6\pm 0.3$&$2.105\pm 0.010$\\
090300120010 & 2010-03-06 18:12:11 &1216&$10.8\pm 0.5$&$2.125\pm 0.014$\\
090200120010 & 2010-03-03 21:25:34 &1055&$9.8\pm 0.5$&$2.109\pm 0.012$\\
083900120010 & 2009-08-27 05:12:35 &1119&$8.3\pm 0.3$&$2.061\pm 0.011$\\
083600120010 & 2009-08-18 10:05:54 &1855&$7.9\pm 0.3$&$2.051\pm 0.010$\\
083500120010 & 2009-08-15 06:45:02 &1890&$7.3\pm 0.2$&$2.025\pm 0.009$\\
083400120010 & 2009-08-12 10:31:36 &1961&$8.0\pm 0.3$&$2.051\pm 0.010$\\
077400120010 & 2009-02-13 18:35:41 &1068&$8.1\pm 0.3$&$2.057 \pm 0.011$\\
072800120010 & 2008-09-29 04:39:52 &1079&$8.1\pm 0.3$&$2.058\pm 0.011$\\
072700120010 & 2008-09-26 04:33:46 &1161& $7.7\pm 0.3$&$2.037\pm 0.011$\\
072301160010 & 2008-09-16 15:28:01 &FAILED&&\\
066600120010 & 2008-03-27 16:50:23 &1096&$7.9\pm 0.3$&$2.049\pm 0.010$\\
066500120010 & 2008-03-24 17:22:19 &FAILED&&\\
060500120010 & 2007-09-27 05:04:15 &1167&$9.1\pm 0.3$& $2.072\pm 0.009$\\
054100120010 & 2007-03-19 18:14:47 &995&$7.6\pm 0.3$&$2.038\pm 0.011$\\
048300410010 & 2006-09-28 17:15:02 &2314&$9.2\pm 0.2$&$2.083\pm 0.006$\\
046800040010 & 2006-08-13 05:01:13 &1346&$7.9\pm 0.2$&$2.051 \pm 0.009$\\
046400490010 & 2006-08-02 21:38:15 &1895&$8.4\pm 0.3$&$2.066\pm 0.11$\\
042800690010 & 2006-04-18 03:47:30 &1320&$9.8\pm 0.4$&$2.104\pm 0.011$\\
042200120010 & 2006-03-28 22:48:25 &1109&$8.7\pm	0.3$ &$2.072\pm 0.009$\\
042000140010 & 2006-03-23 03:16:37 &1435& $9.7\pm 0.3$& $2.091\pm 0.009$\\
037200190010 & 2005-10-30 19:17:40 &1494 &$8.8\pm 0.3$&$2.067\pm 0.009$\\
036500790010 & 2005-10-11 02:29:23 &2544 &$21.4\pm 0.4$&$2.308\pm 0.006$\\
035200120010 & 2005-08-31 19:18:08 &2308 &$16.9\pm 0.4$&$2.241\pm 0.007$\\
030800040010	& 2005-04-21 20:08:30	 &1476&$18.9\pm 0.6$& $2.274\pm 0.008$\\
030100140010 & 2005-04-01 06:04:53 & 1464 &$ 19.7\pm 0.7$& $2.285\pm		0.010$ \\
030000120010 &2005-03-29 16:16:40 &1090&$18.7\pm 0.6$&$2.279\pm		0.009$\\
024200100010 & 2004-10-06 13:50:27 &1509 &$7.0\pm 0.2$&$2.015\pm 0.009$\\
023900120010 & 2004-09-27 17:54:01 & 1356&$8.2\pm 0.2$&$2.062\pm 0.008$\\
022900500010 & 2004-08-29 22:56:58 &1406 &$8.3\pm 0.3$&$2.062	\pm	0.009$\\
022500120010 & 2004-08-16 18:53:43 &1496 &$9.5\pm 0.3$&$2.096\pm 0.009$\\
018200130010 & 2004-04-10 10:58:12&2465 & $8.2\pm 0.2$ &$2.055\pm 0.008$\\
017700170010 & 2004-03-26 11:19:37 & 1584& $7.7\pm 		0.2$& $2.042	\pm	0.008$\\
017000370010 & 2004-03-05 18:20:37 &1431&$9.4		\pm 0.3$& $2.092	\pm	0.009$ \\
012600140010 & 2003-10-25 23:07:59 &2540 &$18.9\pm		0.5$&$2.271\pm 0.008$\\
012500120010 & 2003-10-22 20:14:19 &2552 &$19.8\pm		0.5$&$2.287	\pm 	0.007$\\
012400120010 & 2003-10-19 20:26:07 &2522 &$20.8		\pm 0.5$&$2.295		\pm 0.007$\\
012301100010 & 2003-10-18 20:37:15 &3029 &$18.5		\pm 0.5$ &$2.267\pm 0.009$ \\
010200120010 & 2003-08-15 10:07:51 &1156 &$18.2		\pm 0.5$&$2.267	\pm	0.009$\\
005800240010 & 2003-04-05 17:09:22 &1635 &$7.8		\pm 0.2$&$2.037\pm 0.007$\\
005500820010 & 2003-03-29 05:49:23 &1622 & $9.8\pm 0.3$ &$2.097\pm 0.008$ \\
005100590010 & 2003-03-16 10:09:26 & 1656 &$7.8\pm 0.3$& $2.034\pm 0.009$\\
004700200010 & 2003-03-03 14:12:29 &1581&$9.17 \pm 0.26$  &$2.081\pm 0.008$\\
\hline
\end{tabular}
\end{table*}
\begin{table*}
\begin{tabular}{|l|l|l|l|l|}
\hline
ScW &Start &  Exposure & Flux & $\Gamma$\\
\hline
004500120010 & 2003-02-25 10:17:19 &1525 &$9.2		\pm 0.3$& $2.078\pm 0.010$\\
004400120010 & 2003-02-22 10:45:30 &1572 & $9.3\pm 0.3$& $2.080\pm 0.007$\\
004300120010 & 2003-02-19 20:35:25	& 1281 & $9.12\pm 0.24$ & $2.081\pm 0.008$\\
004200120010 & 2003-02-17 01:25:43 & 2433 & $9.5\pm 0.2$ & $2.091\pm 0.006$\\
004100010050 & 2003-02-13 10:15:23 & 2703 & $9.3\pm 0.3$ & $2.081\pm 0.008$\\
004000060180 & 2003-02-12 12:51:41  & 3190 & $9.1\pm 0.2$&$2.078\pm 0.007$\\
003900020150 & 2003-02-07 22:08:51 &2728 & $8.29\pm 0.16$ & $2.055\pm 0.005$\\
\hline
\end{tabular}
\caption{Data set used for Crab variability analysis. Failed: 836f4dfde420727412db6428a5ba9beb | Job Id : 285ABOR4RBZJ1QMJ;  d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : CA57X71JAI1H3I7T;  89243f581f8dd48a01a9e65019e98259 | Job Id : BBM7N8763XV03MGB;
d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : 2AJPKSH15M1SGFK0;  d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : JBU3UMQ2WKG561IT;89243f581f8dd48a01a9e65019e98259 | Job Id : QQUXNEI5NRJTC7AF; d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : 85CJCHIW5LVU66IN; 836f4dfde420727412db6428a5ba9beb | Job Id : OTZGRFP8H85AJWQT; d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : 4L602VZ8NPP0LADK; d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : 5GD3PP9S3H0Z9BYR; d50b9aa1d7b3c87e1e76e723ec7beaf3 | Job Id : TXCHKYKGD38VL3R9; 89243f581f8dd48a01a9e65019e98259 | Job Id : X0XTRP76OYWXG54U; 836f4dfde420727412db6428a5ba9beb | Job Id : NGBECA9ZO7WSJJ0Y}
\label{tab:crab_scw}
\end{table*}


